Shield Synthesis: Runtime Enforcement for Reactive Systems

Scalability issues may prevent users from verifying critical properties of a complex hardware design. In this situation, we propose to synthesize a "safety shield" that is attached to the design to enforce the properties at run time. Shield synthesis can succeed where model checking and reactive synthesis fail, because it only considers a small set of critical properties, as opposed to the complex design, or the complete specification in the case of reactive synthesis. The shield continuously monitors the input/output of the design and corrects its erroneous output only if necessary, and as little as possible, so other non-critical properties are likely to be retained. Although runtime enforcement has been studied in other domains such as action systems, reactive systems pose unique challenges where the shield must act without delay. We thus present the first shield synthesis solution for reactive hardware systems and report our experimental results. This is an extended version of [5], featuring an additional appendix.

==> figs/odta_example.tex <==
\begin{tikzpicture}[auto,node distance=\nd]
\node[state] at  (0,0)       (m0) {$m_0$};

\path
(m0) edge [loop left]  node 
     {$(o_i=o_i') \textcolor{blue}{\rightarrow 0}$} (m0)
(m0) edge [loop right] node 
     {$(o_i\neq o_i') \textcolor{blue}{\rightarrow 1}$} (m0);
\end{tikzpicture}
% 
